Byzantine Convergence in Robots Networks: The Price of Asynchrony

We study the convergence problem in fully asynchronous, uni-dimensional robot networks that are prone to Byzantine (i.e. malicious) failures. In these settings, oblivious anonymous robots with arbitrary initial positions are required to eventually converge to an a apriori unknown position despite a subset of them exhibiting Byzantine behavior. Our contribution is twofold. We propose a deterministic algorithm that solves the problem in the most generic settings: fully asynchronous robots that operate in the non-atomic CORDA model. Our algorithm provides convergence in 5f+1-sized networks where f is the upper bound on the number of Byzantine robots. Additionally, we prove that 5f+1 is a lower bound whenever robot scheduling is fully asynchronous. This constrasts with previous results in partially synchronous robots networks, where 3f+1 robots are necessary and sufficient.

==> lower_bounds.tex <==
\subsection{Lower bound for byzantine resilient convergence}
\label{sec:lower-bounds}

The following lemma shows that any cautious algorithm needs at least $3f+1$ robots in order to tolerate $f$ byzantine robots in uni-dimensional environments.

\begin{lem}
\label{impossibility-3f-atom}
It is impossible to achieve convergence with a cautious algorithm if $n\leq 3f$ in the ATOM model, where $n$ denotes the number of robots and $f$ denotes the number of Byzantine robots.
\end{lem}

The following corollary provides the lower bound for the CORDA model. 

\begin{cor}
\label{impossibility-3f-corda}
Byzantine-resilient convergence is impossible for $n \leq 3f$ with a cautious algorithm in the CORDA model.
\end{cor}

The following section proves that this bound is tight, the proof is constructive: we give a cautious convergence algorithm that operates correctly in the presence of up to $f$ Byzantine robots provided that the total number of robots is at least $3f+1$, and then we formally prove its correctness.





